Online Distributed Sensor Selection

A key problem in sensor networks is to decide which sensors to query when, in order to obtain the most useful information (e.g., for performing accurate prediction), subject to constraints (e.g., on power and bandwidth). In many applications the utility function is not known a priori, must be learned from data, and can even change over time. Furthermore for large sensor networks solving a centralized optimization problem to select sensors is not feasible, and thus we seek a fully distributed solution. In this paper, we present Distributed Online Greedy (DOG), an efficient, distributed algorithm for repeatedly selecting sensors online, only receiving feedback about the utility of the selected sensors. We prove very strong theoretical no-regret guarantees that apply whenever the (unknown) utility function satisfies a natural diminishing returns property called submodularity. Our algorithm has extremely low communication requirements, and scales well to large sensor deployments. We extend DOG to allow observation-dependent sensor selection. We empirically demonstrate the effectiveness of our algorithm on several real-world sensing tasks.

==> basicAlgorithm.tex <==
%
%
%
%
%
%
%

\section{Approximation Algorithm}
We will now develop an efficient, distributed no-$(1-1/e)$-regret algorithm for online maximization submodular functions.  

\subsection{Centralized Algorithm for Selecting Multiple Sensors}
In principle, we could interpret the sensor selection problem as a
$\binom{n}{k}$-armed bandit problem, and apply existing no-regret
algorithms such as \EXPthree. Unfortunately, this approach does not
scale, since the number of arms grows exponentially with $k$.
However, in contrast to the traditional multiarmed bandit problem,
where the arms are assumed to have independent payoffs, in the sensor
selection case, the payoff function is submodular.  Recently, Streeter
and Golovin showed how this submodularity can be exploited, and
developed a no-$(1-1/e)$-regret algorithm for online maximization of
submodular functions \cite{streeter08}.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
The key idea behind their algorithm, $\text{OG}_{\text{unit}}$, is to
turn the offline greedy algorithm into an online algorithm by
replacing the greedy selection of the element $s_{k}$ that maximizes
the benefit $s_{k}=\argmax_{s} \obj(\{s_{1},...,s_{k-1}\}\cup\{s\})$
by a bandit algorithm. As shown in \ref{}, \OGunit maintains $k$
bandit algorithm, one for each sensor to be selected.  At each round
$t$, $k$ sensors are selected according to the choices of the $k$
bandit algorithms $\Alg_{i}$.  Once the elements have been selected,
the $\ith$ bandit algorithm $\Alg_{i}$ receives as feedback the
incremental benefit
$\obj_{t}(s_{1},\dots,s_{i})-\obj_{t}(s_{1},\dots,s_{i-1})$, i.e., how
much additional utility is obtained by adding sensor $s_{i}$ to the
set of already selected sensors.


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{center}
\begin{tabular}{|p{8cm}|}
\hline
\textbf{Algorithm \OGunit from~\cite{streeter08}:}\\
\hspace{0cm} Initialize $\K$ multiarmed bandit algorithms  $\Alg_1, \Alg_2, \ldots, \Alg_\K$,\\ 
\hspace{0cm} each with action set $\sensors$.\\
\hspace{0cm} For each round $t \in [T]$\\
\hspace{0.3cm} For each stage $i \in [\K]$ in parallel\\
\hspace{0.6cm}      $\Alg_i$ selects an action $\sensor^t_i$\\
\hspace{0.3cm} For each $i \in [\K]$ in parallel\\
\hspace{0.6cm}      feedback $\obj_t(\set{\sensor^t_j : j
  \le i }) - \obj_t(\set{\sensor^t_j : j < i })$ to $\Alg_i$.\\
\hspace{0.3cm} Output $S_t = \set{a^t_1, a^t_2, \ldots, a^t_\K}$.\\
\hline
\end{tabular}
\end{center}

Note that $\text{OG}_{\text{unit}}$ needs only to send the sensor
readings from $\set{\sensor^t_i : i \in [\K]}$ to the server once they
are chosen.  Unfortunately, \EXPthree (and in fact all known
multiarmed bandit algorithms with no-regret guarantees suitable for
use with \OGunit) require sampling from some distribution with weights
associated with the sensors.
%
%
%
%
If $|\sensors|$ is small, we could simply store these weights on the
server, and run the bandit algorithms $\Alg_i$ there.  However, this
solution does not scale to large numbers of sensors.  Thus the key
problem for online sensor selection is to develop a multiarmed bandit
algorithm which implements \emph{distributed sampling} across the
network, with minimal overhead of communication.  In addition, the
algorithm needs to be able to maintain the distributions (the weights)
associated with each $\Alg_{i}$ in a distributed fashion.
%
%
In the following, we will develop novel algorithms that address these
key challenges.
%


\ignore{
\subsection{Overview}
\begin{itemize}
\item Intuitively explain online algorithm and its relationship to greedy algorithm
\item Naive approach requires lots of coordination
\item Key problem: Distributed multinomial sampling
\end{itemize}
}

%
%
%
%
%
%


==> multiSensor.tex <==
%
%
%
%
%
%
%

\commentout{

%
\section{Selecting Multiple Sensors}
\label{sec:single}
%

We will now develop an efficient, distributed no-$(1-1/e)$-regret
algorithm for online maximization submodular functions.  


\subsection{Centralized Selection of Multiple Sensors}
In principle, we could  interpret the sensor selection problem as a $\binom{n}{k}$-armed bandit problem, and apply existing no-regret algorithms such as \EXPthree. Unfortunately, this approach does not scale, since the number of arms grows exponentially with $k$.  However, in contrast to the traditional multiarmed bandit problem, where the arms are assumed to have independent payoffs, in the sensor selection case, the payoff function is submodular.
Recently, Streeter and Golovin showed how this submodularity can be exploited, and
developed a no-$(1-1/e)$-regret algorithm for online maximization of submodular functions \cite{streeter08}. 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
The key idea behind their algorithm, $\text{OG}_{\text{unit}}$, is to turn the offline greedy algorithm into an online algorithm by replacing the greedy selection of the element $s_{k}$ that maximizes the benefit $s_{k}=\argmax_{s} \obj(\{s_{1},...,s_{k-1}\}\cup\{s\})$ by a bandit algorithm. As shown in \ref{}, \OGunit maintains $k$ bandit algorithm, one for each sensor to be selected.  At each round $t$, $k$ sensors are selected according to the choices of the $k$ bandit algorithms $\Alg_{i}$.  Once the elements have been selected, the $i$-th bandit algorithm $\Alg_{i}$ receives as feedback the incremental benefit $\obj_{t}(s_{1},\dots,s_{i})-\obj_{t}(s_{1},\dots,s_{i-1})$, i.e., how much additional utility is obtained by adding sensor $s_{i}$ to the set of already selected sensors.


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{center}
\begin{tabular}{|p{8cm}|}
\hline
\textbf{Algorithm \OGunit from~\cite{streeter08}:}\\
\hspace{0cm} Initialize $\K$ multiarmed bandit algorithms  $\Alg_1, \Alg_2, \ldots, \Alg_\K$,\\ 
\hspace{0cm} each with action set $\sensors$.\\
\hspace{0cm} For each round $t \in [T]$\\
\hspace{0.3cm} For each stage $i \in [\K]$ in parallel\\
\hspace{0.6cm}      $\Alg_i$ selects an action $\sensor^t_i$\\
\hspace{0.3cm} For each $i \in [\K]$ in parallel\\
\hspace{0.6cm}      feedback $\obj_t(\set{\sensor^t_j : j
  \le i }) - \obj_t(\set{\sensor^t_j : j < i })$ to $\Alg_i$.\\
\hspace{0.3cm} Output $S_t = \set{a^t_1, a^t_2, \ldots, a^t_\K}$.\\
\hline
\end{tabular}
\end{center}

Theorem~$12$ of~\cite{streeter07tr} states that \OGunit has a
$\paren{1-\frac{1}{e}}$-regret bound of $O(\K \sqrt{T n \log n})$, in this (partially-transparent) feedback model.


Note that \OGunit needs only to send the sensor
readings from $\set{\sensor^t_i : i \in [\K]}$ to the server once they
are chosen, and uses the multiarmed bandit algorithms in a quite
modular fashion.  This makes it a suitable foundation for building a
distributed algorithm, given the distributed multiarmed bandit
algorithm described in~\secref{sec:single}.



\dan{ Move or delete this?}
\textit{
Unfortunately, \EXPthree (and in fact all known multiarmed bandit
algorithms with no-regret guarantees suitable for use with \OGunit)
require sampling from some distribution with weights associated with
the sensors.
%
%
%
%
If $\numsensors$ is small, we could simply store these weights on the
server, and run the bandit algorithms $\Alg_i$ there.  However, this
solution does not scale to large numbers of sensors.  Thus the key
problem for online sensor selection is to develop a multiarmed bandit
algorithm which implements \emph{distributed sampling} across the
network, with minimal overhead of communication.  In addition, the
algorithm needs to be able to maintain the distributions (the weights)
associated with each $\Alg_{i}$ in a distributed fashion.
%
%
In the following, we will develop novel algorithms that address these key challenges. 
%
}

}

==> overview.tex <==
\section{Overview of our approach}\label{sec:overview}
In the following Sections, we will develop our Distributed Online
Greedy (\dog) algorithm for distributed online selection of sensors.
In \secref{sec:centralized}, we will first discuss how the greedy
algorithm for a known objective function can be extended to an online
algorithm with no-$(1-1/e)$-regret.  The key step is to replace each
greedy selection step with a multiarmed bandit algorithm. In
\secref{sec:distributed}, we will then show how the online algorithm
from \secref{sec:centralized} can be implemented efficiently in a
distributed manner. A primary consideration in devising the protocol
is the cost of sending messages between sensors and the base station.
We consider two cost models.
\begin{itemize}
\item In the \emph{broadcast} model, each sensor can broadcast a
message to all other sensors at unit cost.
\item In the \emph{star network} model, messages can only be between
  two sensors or a sensor and the base station, and each message has
  unit cost. \matt{As stated, this is just multi-hop. Are messages
  between two sensors allowed?}
\end{itemize}
In \secref{sec:distributed} we first consider the broadcast model, and
then show how it can be extended to the star network model in
\secref{sec:lazy-renorm}. In \secref{sec:measure-dependent-sampling},
we will then extend our algorithm to allow for observation-specific
selection.


%
%
%
%
%
%


==> sampling.tex <==
%
%
%
%
%
%
%

\subsection{Distributed Multinomial Sampling} \label{sec:sampling}

A key subproblem in the design of our algorithm is the ability to
sample exactly one element from a probability distribution $p$ over
sensors.  We wish to do so in as distributed a manner as possible.
We assume that each sensor $\sensor \in \sensors$ stores its probability mass $p_\sensor$ with
it, and can send messages to and receive messages from a central
server.  The central server should not need to know the distribution
$p$.  Though the existence of such a server means the protocol is not
completely distributed, it is realistic in sensor network applications
where the sensor data needs to be accumulated somewhere for analysis.
We also assume the sensors have calibrated clocks.
We measure the cost of the sampling procedure in terms of the number
of messages transmitted, where each message is a constant number of
words, or $\cO(\log n)$ bits where $n = |\sensors|$.


A completely centralized solution would have each sensor $\sensor$
simply transmit $p_{\sensor}$ to the server, which would then make the
selection.  This requires $n$ messages.  In this section we present a
protocol that requires only $\cO(\log n)$ messages with high
probability, and a variant that requires only $\cO(1)$ messages to
select at most one sensor where each sensor is selected with
probability proportional to its original mass. 

\begin{theorem} \label{thm:sampling}
There exists a protocol for selecting exactly one sensor according to
any fixed distribution $p$ such that with high probability the number
of messages required is $\cO(\log n)$.  Moreover, for all $\alpha \ge
1$, there exists a protocol for selecting at most one sensor such that 
$\prob{\sensor \text{ selected}} = (1 - e^{-\alpha})p_{\sensor}$ which
requires no more than $\alpha$ messages in expectation.
\end{theorem}

We devote the rest of the section to proving
Theorem~\ref{thm:sampling}.  For a sampling procedure with input
distribution $p$, we let $\psamp$ denote the resulting distribution,
where in all cases at most one sensor is selected, and nothing is
selected with probability $1-\sum_{\sensor} p_{\sensor}$.
We start with the following simple protocol that does not satisfy the
guarantees of Theorem~\ref{thm:sampling}.

\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The Simple Protocol:}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Bernoulli{p_{\sensor}}$.\\
\hspace{0.5cm} If $(X_{\sensor} = 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else select a sensor uniformly at random from $S$.\\
\hline
\end{tabular}
\end{center}

It is not hard to show that for all sensors $\sensor$, 
\[
\psamp_{\sensor} = p_{\sensor}\cdot \Econd{\frac{1}{|S|}}{\sensor \in S} \ge p_{\sensor}/ \Econd{|S|}{\sensor \in S} \ge
p_{\sensor}/2 
\] 
by appealing to Jensen's inequality.
Since $\psamp_{\sensor} \le p_{\sensor}$, we find that this simple
protocol maintains a ratio $r_{\sensor} := \psamp_{\sensor} /
p_{\sensor} \in [\frac12 , 1]$.  Unfortunately, this analysis is
tight, as can be seen from an example with two sensors with
$p_1 = \eps, p_2  = 1 - \eps$.


To improve upon the simple protocol, first consider running it on an example
with $p_1 = p_2 = \cdots = p_n = 1/n$.  Since the protocol behaves
exactly the same under permutations of sensor labels, by symmetry we
have $\psamp_{1} = \psamp_{2} = \cdots = \psamp_{n}$, and thus 
$r_i = r_j$ for all $i,j$.  Now consider an input distribution $p$
where there exists integers $N$ and $k_1, k_2, \ldots, k_n$ such that 
$p_{\sensor} = k_{\sensor}/N$ for all $\sensor$.
Replace each $\sensor$ with $k_{\sensor}$ fictitious sensors, each with
probability mass $1/N$, and each with a label indicating $\sensor$.
Run the simple protocol with the fictitious sensors, selecting a fictitious sensor
$\sensor'$, and then actually select the sensor indicated by the label
of $\sensor'$.
By symmetry this process selects each fictitious sensor with probability $(1-\eta)/N$,
where $\eta$ is the probability that nothing at all is selected, and
thus the process selects sensor $\sensor$ with probability 
$k_{\sensor}(1-\eta)/N = (1-\eta)p_{\sensor}$
(since at most one fictitious sensor is ever selected).



We may thus consider the following improved protocol which
incorporates the above idea, simulating this modification to the
protocol exactly when $p_{\sensor} = k_{\sensor}/N$ for all $\sensor$.

\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The Improved Protocol($N$):}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Binomial{\ceil{N \cdot
    p_{\sensor}}, 1/N}$.\\
\hspace{0.5cm} If $(X_{\sensor} \ge 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else, select $\sensor$ with probability
$X_{\sensor}/\sum_{\sensor' \in S} X_{
\sensor'}$.\\
\hline
\end{tabular}
\end{center}

This protocol ensures the ratios $r_{\sensor} := \psamp_{\sensor} /
p_{\sensor}$ are the same for all sensors, provided each $p_{\sensor}$
is a multiple of $1/N$.  Assuming the probabilities are rational,
there will be a sufficiently large $N$ to satisfy this condition.
To reduce $\eta := \prob{S = \emptyset}$ in the simple protocol, we
may sample each $X_{\sensor}$ from $\Bernoulli{\alpha/n}$ for any
$\alpha \in [1, n]$.  The symmetry argument remains unchanged.
This in turn suggests sampling $X_{\sensor}$ from 
$\Binomial{\ceil{N \cdot p_{\sensor}}, \alpha/N}$ in the improved
protocol.  Taking the limit as $N \to \infty$, the binomial
distribution becomes Poisson, and we obtain the desired protocol.


\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The \LimitProtocolns($\alpha$):}\\
\hspace{0cm} Same as the improved protocol, except each \\ 
\hspace{0cm} sensor $\sensor$ samples $X_{\sensor} \sim \Poisson{\alpha p_{\sensor} }$\\
\ignore{
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Poisson{\alpha p_{\sensor} }$.\\
\hspace{0.5cm} If $(X_{\sensor} \ge 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else, select $\sensor$ with probability
$X_{\sensor}/\sum_{\sensor' \in S} X_{\sensor'}$.\\
}
\hline
\end{tabular}
\end{center}

Straight-forward calculation shows that 
\begin{align}
\prob{S = \emptyset}  
%
& = \prod_{\sensor} \exp\set{ - \alpha \cdot p_{\sensor}} \\
& = \exp \curlyparen{ - \sum_{\sensor} \alpha \cdot p_{\sensor}} \\
& = \exp \set{-\alpha}   
\end{align}
Let $C$ be the number of messages sent to the server.  Then 
\begin{align}
\E{C} & =  \sum_{\sensor} \prob{X_{\sensor} \ge 1} \\
 & = \sum_{\sensor} (1-\exp\set{-\alpha p_{\sensor}})\\
 & \le  \sum_{\sensor} \alpha p_{\sensor} \\
 & = \alpha\mbox{.}
\end{align}
Here we have used linearity of expectation in the first line, and $1+x
\le e^x$ for all $x \in \Real$ in the third.
This completes the proof of the second part of
Theorem~\ref{thm:sampling}.
To prove the first part, and ensure we always select some sensor, it
suffices to set $\alpha = \ln(n)$ and in the unlikely event that $S =
\emptyset$, simply have the server broadcast a command to all sensors
to rerun the protocol with fresh random seeds as many times as needed
until $S$ is non-empty. 

%
\subsection{Activation in the Broadcast Model}
%

\begin{prop}
Rerunning the \LimitProtocol until an
element is selected results in at most  $\alpha / (1 - e^{-\alpha})$
%
elements being activated in expectation.  Moreover, this value is tight.
\end{prop}

\begin{proof}
Let $X_{\sensor} \sim \Bernoulli{\alpha \cdot p_{\sensor}}$ be the indicator random
variable for the activation of $\sensor$, and let $X := \sum_{\sensor}
X_{\sensor}$.  The expected number of sensor activations is then
\[
\E{X \ |\ X \ge 1} = \E{X}/\prob{X \ge 1} \mbox{.}
\]
In the limit as $\max_{\sensor} p_{\sensor}$ tends to zero, $X$
converges to a Poisson random variable with mean $\alpha$.
In this case, $\frac{\E{X}}{\prob{X \ge 1}} = \alpha / (1 - e^{-\alpha})$
To see that this is an upper bound, consider an arbitrary distribution
$p$ on the sensors, and fix some $\sensor$ with $x := p_{\sensor} > 0$.
We claim that replacing $\sensor$ with two sensors $\sensor_1$ and
$\sensor_2$ with positive probability mass $x_1$ and
$x_2$ with $x = x_1+x_2$ can only serve to increase the expected number of
sensor activations, because $\E{X}$ is unchanged, and $\prob{X \ge 1}$
decreases.  The latter is true essentially because 
$\prob{\exists i \in \set{1,2}: \sensor_i \text{ activates}} = 1 -
(1-x_1)(1-x_2) = x - x_1x_2 < x$.  To complete the proof, notice that 
repeating this process with $\sensor = \argmax (p_{\sensor})$ and $x_i = x/2$ ensures $X$
converges to a Poisson variable with mean $\alpha$, while only
increasing $\E{X \ |\ X \ge 1}$.
\ignore{
easily verified by noting that conditioning
on the event $\event$ that no sensors in $\sensors \setminus
\set{\sensor, \sensor_1, \sensor_2}$ activate, $\prob{\sensor \text{ activates} | \event} = x$ and 
$\prob{\exists i \in \set{1,2}: \sensor_i \text{ activates} | \event} = 1 -
(1-x_1)(1-x_2) = x - x_1x_2 < x$.
}
\end{proof}



%
\subsection{Lazy Renormalization} \label{sec:lazy-renorm}
%

Multiarmed bandit algorithms maintain a distribution over actions, and
update this distribution in response to feedback about the environment.
Often the mass of all actions will be affected in each round via
a renormalization step.  Certain MAB algorithms allow this step to be
computed in a semi-distributed manner.  For example, \EXPthree~\cite{auer02}
maintains weights $w_\sensor(t)$ for all actions $\sensor$ and all
  times $t$, and samples $\sensor$ with probability 
$p_{\sensor}(t) :=
  (1-\gamma)w_\sensor(t)/\sum_{\sensor'}w_{\sensor'}(t) +
  \gamma/|\sensors|$, where $\gamma$ is an input parameter.
In each round only the one selected action $\sensor$ has its weight
updated.  If it's reward is $\payoff(\sensor, t)$ the update is 
$w_{\sensor}(t+1) = w_{\sensor}(t)\exp\paren{\frac{\gamma}{|\sensors|}\frac{\payoff(\sensor,
    t)}{p_{\sensor}(t)}}$.  For all other actions $\sensor'$, 
$w_{\sensor'}(t+1) = w_{\sensor'}(t)$.
This means that each sensor $\sensor$ requires only $w_{\sensor}(t)$
and $\sum_{\sensor'}w_{\sensor'}(t)$ to compute $p_{\sensor}(t)$.
The former changes only when $\sensor$ is selected.
In the broadcast model the latter can simply be broadcast at the end
of each round, however things are not so easy in the star network model.
Nevertheless, in this section we show that under certain assumptions
(which hold true for \EXPthree) we can perform the
necessary renormalization in a lazy manner, while still keeping the
amount of communication quite low.


Our lazy renormalization scheme works as follows.
Each sensor $\sensor$ maintains its weight $w_{\sensor}(t)$ and
estimate $W_{\sensor}(t)$ for $W(t) :=
\sum_{\sensor'}w_{\sensor'}(t)$, 
Initially, $W_{\sensor}(0) = |\sensors|$. 
The central server stores $W(t)$ for all previous rounds $t$.
Each sensor then proceeds with the sampling procedure of
section~\ref{sec:sampling} as though its probability mass in round $t$
was $p_{\sensor} = w_{\sensor}(t)/W_{\sensor}(t)$ instead of its true
value of $w_{\sensor}(t)/W(t)$.  Moreover, $\sensor$'s estimate 
$W_{\sensor}(t)$ is only updated on rounds when it communicates with
the server under these circumstances.  This allows the estimated
probabilities of all of the sensors to sum to more than one, but has
the benefit of significantly reducing the communication cost in the
star network model under certain assumptions.  The protocol for round $t$ is as follows.

\begin{center}
\begin{tabular}{|p{8cm}|}
\hline
\textbf{The \LimitProtocol($\alpha$) with renormalization:}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $r_{\sensor}$ uniformly at random from $[0,1]$.\\
\hspace{0.5cm} If $(r_{\sensor} \ge 1 - \alpha \cdot w_{\sensor}(t) / W_{\sensor}(t))$\\
\hspace{1cm} Send $\tuple{r_{\sensor}, w_{\sensor}(t)}$ to the server.\\ 
\hspace{1cm} Receive message $\tuple{a, b}$ from server.\\
\hspace{1cm} Set $W_{\sensor}(t+1) = a$, $w_{\sensor}(t+1) = b$. \\
\hspace{0.5cm} Else\\
\hspace{1cm} Set $W_{\sensor}(t+1) = W_{\sensor}(t)$, $w_{\sensor}(t+1) = w_{\sensor}(t)$.\\
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing and wait for next round.\\
\hspace{0cm} Else\\
\hspace{0.5cm} For each sensor $\sensor \in S$\\
\hspace{1cm} Set $Y_{\sensor} = \min \set{x : \prob{X \le x} \ge r}$, \\
\hspace{1cm} where $X \sim \Poisson{\alpha \cdot w_{\sensor}(t)/W(t)}$.\\
%
%
%
\hspace{1cm} Select $\sensor$ with probability
$Y_{\sensor}/\sum_{\sensor' \in S} Y_{\sensor'}$.\\
\hspace{0.5cm} Observe the payoff and compute $W(t+1)$\\
\hspace{0.5cm} and $w_{\sensor}(t+1)$ for each $\sensor \in S$.\\
\hspace{0.5cm} For each $\sensor \in S$, send $\tuple{W(t+1), w_{\sensor}(t+1)}$ to $\sensor$.\\
\hline
\end{tabular}
\end{center}


We now describe the assumptions that allow lazy renormalization to
have low communication costs.
Fix an action $\sensor$ and a multiarmed bandit algorithm.
Let $p_{\sensor}(t) \in [0,1]$ be random variables denoting the
probability the algorithm assigns to $\sensor$ on round $t$.
The value of $p_{\sensor}(t)$ depends on the random choices made by
the algorithm and the payoffs observed by it on previous rounds.
We assume the following about $p_{\sensor}(t)$.
\begin{enumerate}
\item There exists an $\epsilon > 0$ such that $p_{\sensor}(t)
  \ge \epsilon$ for all $t$.
\item $p_{\sensor}(t) < p_{\sensor}(t+1)$ implies $\sensor$ was
  selected in round $t$.
\item There exists $\hat{\epsilon} > 0$ such that 
  $p_{\sensor}(t+1) \ge p_{\sensor}(t)/(1+\hat{\epsilon})$ for all $t$.
\end{enumerate}
Many MAB algorithms satisfy these conditions.
For example, it is not too difficult to show \EXPthree does so 
with $\epsilon = \gamma/|\sensors|$ and
$\hat{\epsilon} = (e-1)\frac{\gamma}{|\sensors|}$, assuming payoffs in $[0,1]$.
In this case, Theorem~\ref{thm:lazy_renorm_ratio} bounds the expected
increase in sensor communications due to lazy renormalization.
%
%
%

\begin{theorem} \label{thm:lazy_renorm_ratio}
Fix a multiarmed bandit instance with possibly adversarial payoff
functions, and a MAB algorithm 
%
satisfying the above assumptions on its distribution over actions
$\set{p_{\sensor}(t)}_{\sensor \in \sensors}$.
Let $q_{\sensor}(t)$ be the corresponding random estimates for
$p_{\sensor}(t)$ maintained under lazy renormalization with
oversampling parameter $\alpha$.
Then for all $\sensor$ and $t$, 
\[
\E{q_{\sensor}(t)/p_{\sensor}(t)} \le 1 + \frac{\hat{\epsilon}}{\alpha\epsilon}
\mbox{.}
\]
\end{theorem}


\begin{proof}
Fix $\sensor$, and let $p(t) := p_{\sensor}(t)$, $q(t) := q_{\sensor}(t)$.
We begin by bounding $\prob{q(t) \ge \lambda p(t)}$ for $\lambda \ge
1$.  Let $t_0$ be the most recent round in which $q(t_0) = p(t_0)$.
We assume $q(0) = p(0)$, so $t_0$ exists.
Then $q(t) = p(t_0) \ge \lambda p(t)$  implies $p(t_0)/p(t)
\ge \lambda$.  By assumption $p(t')/p(t'+1) \le (1+\hat{\epsilon})$
for all $t'$, so $p(t_0)/p(t) \le (1+\hat{\epsilon})^{t-t_0}$.
Thus $\lambda \le (1+\hat{\epsilon})^{t-t_0}$ and 
$t-t_0 \ge \ln(\lambda)/ \ln (1+\hat{\epsilon})$. 
Define $t(\lambda) := \ln(\lambda)/ \ln (1+\hat{\epsilon})$.


By definition of $t_0$, there were no activations under lazy renormalization in rounds $t_0$
through $t-1$ inclusive, which occurs with probability 
$\prod_{t' = t_0}^{t-1} (1-\alpha q(t'))$ $=$ $(1-\alpha
q(t))^{t-t_{0}} $ $\le$ $(1-\alpha q(t))^{\ceil{t(\lambda)}}$, where $\alpha$ is the
oversampling parameter in the protocol.  
%
%
We now bound $\Econd{q(t)/p(t)}{q(t)}$.
Recall that $\E{X} = \int_{x = 0}^{\infty} \prob{X \ge x}dx$ for any non-negative
random variable $X$.  It will also be convenient to define 
$\lamexp := \ln(1/(1 - \alpha q(t))) / \ln(1+\hat{\epsilon})$ and assume for now
that $\lamexp > 1$.
Conditioning on $q(t)$, we see that 
\[
\begin{array}{lcl}
 \vspace{2mm}
\Econd{q(t)/p(t)}{q(t)} & = & \int_{\lambda = 0}^{\infty} \prob{q(t) \ge
  \lambda p(t)}d\lambda \\ 
 \vspace{2mm}
  & = & 1 + \int_{\lambda = 1}^{\infty} \prob{q(t) \ge
  \lambda p(t)}d\lambda \\ 
\vspace{2mm}
 & \le & 1 + \int_{\lambda = 1}^{\infty} (1-\alpha q(t))^{t(\lambda)}d\lambda\\
 \vspace{2mm}
 & = & 1 + \int_{\lambda = 1}^{\infty}
\lambda^{\ln(1-\alpha q(t))/\ln(1+\hat{\epsilon}) }d\lambda \\
 \vspace{2mm}
 & = & 1 + \int_{\lambda = 1}^{\infty} \lambda^{-\lamexp}d\lambda \\ 
 \vspace{2mm}
 & = & 1 + \frac{1}{\lamexp - 1}
%
%
\end{array}
\]
Using $\ln\paren{\frac{1}{1-x}} \ge x$ for all $x < 1$ and 
$\ln(1+x) \le x$ for all $x > -1$, we can show that 
%
%
$\lamexp \ge \alpha q(t)/\hat{\epsilon}$
so $1+\frac{1}{\lamexp - 1} \le \alpha
q(t)/(\alpha q(t) - \hat{\epsilon})$.
Thus, if $\alpha q(t) > \hat{\epsilon}$ then $\lamexp > 1$ and we
obtain 
$\Econd{q(t)/p(t)}{q(t)} \le  \alpha q(t)/(\alpha q(t) - \hat{\epsilon})$.


If $q(t) >> \hat{\epsilon}$, this gives a good bound.  If $q(t)$ is small, we
rely on the assumption that $p(t) \ge \epsilon$ for all $t$ to get a trivial
bound of $q(t)/p(t) \le q(t)/\epsilon$.
We thus conclude 
$\Econd{q(t)/p(t)}{q(t)} \le \min \paren{\alpha q(t)/(\alpha q(t) - \hat{\epsilon}) ,\ q(t)/\epsilon}$.
Setting $q(t) = (\hat{\epsilon}/\alpha + \epsilon)$ to maximize this
quantity yields an unconditional bound of 
%
%
$\E{q(t)/p(t)} \le 1 + \hat{\epsilon}/\alpha\epsilon$.
\end{proof}


\begin{cor}
Under the above assumptions on $p_{\sensor}(t)$, if \EXPthree is used
with payoffs in $[0,1]$ then $\E{q_{\sensor}(t)/p_{\sensor}(t)} \le 1 + (e-1)/\alpha$.
\end{cor}


%
%
%
%
%
%


==> singleSensor.tex <==
%
%
%
%
%
%
%

\commentout{

%
\section{Distributed Online Selection -- The Single Sensor Case}
\label{sec:single}
%

We will now develop a distributed algorithm for online sensor
selection which is guaranteed to achieve no $(1-1/e)$-regret.  Our
strategy will be to convert the greedy algorithm for centralized
sensor selection for known submodular functions as introduced in
\secref{} into a distributed online algorithm.  As we will show, the
key problem will be to develop an algorithm for selecting a
\emph{single} sensor.  In \secref{} we will then present our algorithm
for selecting multiple sensors, which relies on the single sensor case
as a subroutine.

\subsection{Centralized Online  Single Sensor Selection} \label{sec:centralized-sampling}
Let us first consider the case where $k=1$, i.e., we would like to
select one sensor at each round.  This simpler problem can be
interpreted as an instance of the multiarmed bandit problem (as
introduced in \secref{sec:online-problem}), where we have one arm for
each possible sensor.  If we allow centralized solutions, we can use
no-regret algorithms such as the \EXPthree algorithm \cite{auer02} to
obtain a no-regret sensor selection.  \EXPthree works as follows: It
is parametrized by a \emph{learning rate} $\eta$, and an
\emph{exploration probability} $\gamma$. It maintains a set of weights
$w_{s}$, one for each arm (sensor) $s$, initialized to
1. \andreas{include pseudo-code for \EXPthree?} At every round $t$, it
will select an arm with probability
$$p_{s}=(1-\gamma)\frac{w_{s}}{\sum_{s'}
  w_{s'}}+\frac{\gamma}{\numsensors},$$ i.e., with probability $\gamma$
it explores, picking an arm uniformly at random, and with probability
$(1-\gamma)$ it exploits, picking an arm $s$ with probability
proportional to its weight $w_{s}$.  Once an arm $s$ has been
selected, a feedback $r$ is obtained, and the weight $s_{s}$ is
updated to
$$w_{s}\leftarrow w_{s}\exp(\eta r/p_{s}).$$ Auer et al.~showed that
with appropriately chosen learning rate $\eta$ and exploration
probability $\gamma$ it holds that for the cumulative regret $R_{T}$ of
\EXPthree it holds that $R_{T}=\cO(\sqrt{\numsensors T})$, i.e., the
average regret converges to zero.


If we wish to implement a distributed variant of \EXPthree, there are
two questions we must answer, namely, how do we sample arms and
how do we update the distribution on arms?  We provide answers in
sections~\ref{sec:sampling} and~\ref{sec:lazy-renorm}, respectively,
and prove the following.

\begin{theorem} \label{thm:distributed-single-sensor-selection}
For every $\alpha \in [1, \infty)$ there is a protocol for the
  multiarmed bandit problem such that the worst case expected regret
  is
$O(\sqrt{\OPT \numsensors \log \numsensors} + \OPT e^{-\alpha})$, where
  $\OPT$ is the total reward of the best action, and in each round at most 
$\alpha\paren{1 + (e-1)/\alpha}$ sensors communicate with the server and at most 
$2\alpha\paren{1 + (e-1)/\alpha}$ messages are exchanged in
expectation.
Moreover, there is a protocol with worst case expected regret
$O(\sqrt{\OPT \numsensors \log \numsensors})$ and in each round 
only $O(\log \numsensors)$ sensors  communicate with the server and 
$O(\log \numsensors)$ messages are exchanged with high probability.
\end{theorem}


\subsection{Distributed Multinomial Sampling} \label{sec:sampling}

A key subproblem in the design of our algorithm is the ability to
sample exactly one element from a probability distribution $p$ over
sensors.  We wish to do so in as distributed a manner as possible. We make the following assumptions
\begin{itemize}
\item  Each sensor $\sensor \in \sensors$ stores its probability mass $p_\sensor$ with
it, and can send messages to and receive messages to the base station.  
\item The base station is able, after receiving messages from a set $S$ of sensors, to compute the utility $\obj_{t}(S)$ and send this utility back to the active sensors.  
%
%
\footnote{Though the existence of such a base station means the protocol is not
completely distributed, it is realistic in sensor network applications
where the sensor data needs to be accumulated somewhere for analysis.}
\item The sensors have calibrated clocks.
\end{itemize}
We measure the cost of the sampling procedure in terms of the number
of messages transmitted, where each message is a constant number of
words, or $O(\log n)$ bits where $n = |\sensors|$.


A completely centralized solution would have each sensor $\sensor$
simply transmit $p_{\sensor}$ to the server, which would then make the
selection.  This requires $n$ messages.  In this section we present a
protocol that requires only $O(\log n)$ messages with high
probability, and a variant that requires only $O(1)$ messages to
select at most one sensor where each sensor is selected with
probability proportional to its original mass. 

\begin{theorem} \label{thm:sampling}
There exists a protocol for selecting exactly one sensor according to
any fixed distribution $p$ such that with high probability the number
of messages required is $O(\log n)$.  Moreover, for all $\alpha \ge
1$, there exists a protocol for selecting at most one sensor such that 
$\prob{\sensor \text{ selected}} = (1 - e^{-\alpha})p_{\sensor}$ which
requires no more than $\alpha$ messages in expectation.
\end{theorem}

We devote the rest of the section to proving
Theorem~\ref{thm:sampling}.  For a sampling procedure with input
distribution $p$, we let $\psamp$ denote the resulting distribution,
where in all cases at most one sensor is selected, and nothing is
selected with probability $1-\sum_{\sensor} p_{\sensor}$.
We start with the following simple protocol that does not satisfy the
guarantees of Theorem~\ref{thm:sampling}.

\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The Simple Protocol:}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Bernoulli{p_{\sensor}}$.\\
\hspace{0.5cm} If $(X_{\sensor} = 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else select a sensor uniformly at random from $S$.\\
\hline
\end{tabular}
\end{center}

It is not hard to show that for all sensors $\sensor$, 
\[
\psamp_{\sensor} = p_{\sensor}\cdot \Econd{\frac{1}{|S|}}{\sensor \in S} \ge p_{\sensor}/ \Econd{|S|}{\sensor \in S} \ge
p_{\sensor}/2 
\] 
by appealing to Jensen's inequality.
Since $\psamp_{\sensor} \le p_{\sensor}$, we find that this simple
protocol maintains a ratio $r_{\sensor} := \psamp_{\sensor} /
p_{\sensor} \in [\frac12 , 1]$.  Unfortunately, this analysis is
tight, as can be seen from an example with two sensors with
$p_1 = \eps, p_2  = 1 - \eps$.


To improve upon the simple protocol, first consider running it on an example
with $p_1 = p_2 = \cdots = p_n = 1/n$.  Since the protocol behaves
exactly the same under permutations of sensor labels, by symmetry we
have $\psamp_{1} = \psamp_{2} = \cdots = \psamp_{n}$, and thus 
$r_i = r_j$ for all $i,j$.  Now consider an input distribution $p$
where there exists integers $N$ and $k_1, k_2, \ldots, k_n$ such that 
$p_{\sensor} = k_{\sensor}/N$ for all $\sensor$.
Replace each $\sensor$ with $k_{\sensor}$ fictitious sensors, each with
probability mass $1/N$, and each with a label indicating $\sensor$.
Run the simple protocol with the fictitious sensors, selecting a fictitious sensor
$\sensor'$, and then actually select the sensor indicated by the label
of $\sensor'$.
By symmetry this process selects each fictitious sensor with probability $(1-\eta)/N$,
where $\eta$ is the probability that nothing at all is selected, and
thus the process selects sensor $\sensor$ with probability 
$k_{\sensor}(1-\eta)/N = (1-\eta)p_{\sensor}$
(since at most one fictitious sensor is ever selected).



We may thus consider the following improved protocol which
incorporates the above idea, simulating this modification to the
protocol exactly when $p_{\sensor} = k_{\sensor}/N$ for all $\sensor$.

\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The Improved Protocol($N$):}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Binomial{\ceil{N \cdot
    p_{\sensor}}, 1/N}$.\\
\hspace{0.5cm} If $(X_{\sensor} \ge 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else, select $\sensor$ with probability
$X_{\sensor}/\sum_{\sensor' \in S} X_{
\sensor'}$.\\
\hline
\end{tabular}
\end{center}

This protocol ensures the ratios $r_{\sensor} := \psamp_{\sensor} /
p_{\sensor}$ are the same for all sensors, provided each $p_{\sensor}$
is a multiple of $1/N$.  Assuming the probabilities are rational,
there will be a sufficiently large $N$ to satisfy this condition.
To reduce $\eta := \prob{S = \emptyset}$ in the simple protocol, we
may sample each $X_{\sensor}$ from $\Bernoulli{\alpha/n}$ for any
$\alpha \in [1, n]$.  The symmetry argument remains unchanged.
This in turn suggests sampling $X_{\sensor}$ from 
$\Binomial{\ceil{N \cdot p_{\sensor}}, \alpha/N}$ in the improved
protocol.  Taking the limit as $N \to \infty$, the binomial
distribution becomes Poisson, and we obtain the desired protocol.


\begin{center}
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{The \LimitProtocol($\alpha$):}\\
\hspace{0cm} Same as the improved protocol, except each \\ 
\hspace{0cm} sensor $\sensor$ samples $X_{\sensor} \sim \Poisson{\alpha p_{\sensor} }$\\
\ignore{
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $X_{\sensor} \sim \Poisson{\alpha p_{\sensor} }$.\\
\hspace{0.5cm} If $(X_{\sensor} \ge 1)$, send $X_{\sensor}$ to the server.\\ 
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing.\\
\hspace{0cm} Else, select $\sensor$ with probability
$X_{\sensor}/\sum_{\sensor' \in S} X_{\sensor'}$.\\
}
\hline
\end{tabular}
\end{center}

Straight-forward calculation shows that 
\begin{align}
\prob{S = \emptyset}  
%
& = \prod_{\sensor} \exp\set{ - \alpha \cdot p_{\sensor}} \\
& = \exp \curlyparen{ - \sum_{\sensor} \alpha \cdot p_{\sensor}} \\
& = \exp \set{-\alpha}   
\end{align}
Let $C$ be the number of messages sent to the server.  Then 
\begin{align}
\E{C} & =  \sum_{\sensor} \prob{X_{\sensor} \ge 1} \\
 & = \sum_{\sensor} (1-\exp\set{-\alpha p_{\sensor}})\\
 & \le  \sum_{\sensor} \alpha p_{\sensor} \\
 & = \alpha\mbox{.}
\end{align}
Here we have used linearity of expectation in the first line, and $1+x
\le e^x$ for all $x \in \Real$ in the third.
This completes the proof of the second part of
Theorem~\ref{thm:sampling}.
To prove the first part, and ensure we always select some sensor, it
suffices to set $\alpha = \ln(n)$ and in the unlikely event that $S =
\emptyset$, simply have the server broadcast a command to all sensors
to rerun the protocol with fresh random seeds as many times as needed
until $S$ is non-empty. 




%
\subsection{Lazy Renormalization} \label{sec:lazy-renorm}
%

All multiarmed bandit algorithms with no-regret guarantees against
arbitrary reward functions must maintain a distribution over actions, and
update this distribution in response to feedback about the environment.
Often the mass of all actions will be affected in each round via
a renormalization step.  Certain MAB algorithms allow this step to be
computed in a semi-distributed manner.  
Consider \EXPthree~\cite{auer02}, whose sampling and update procedures
are described in~\secref{sec:centralized-sampling}.
Each sensor $\sensor$ requires only $w_{\sensor}(t)$
and $\sum_{\sensor'}w_{\sensor'}(t)$ to compute $p_{\sensor}(t)$.
The former changes only when $\sensor$ is selected.
In the broadcast model the latter can simply be broadcast at the end
of each round, however things are not so easy in the star network model.
Nevertheless, in this section we show that for \EXPthree (and many
algorithms like it), we can perform the
necessary renormalization in a lazy manner, while keeping the
amount of communication quite low.


Our lazy renormalization scheme for \EXPthree works as follows.
Each sensor $\sensor$ maintains its weight $w_{\sensor}(t)$ and
estimate $W_{\sensor}(t)$ for $W(t) := \sum_{\sensor'}w_{\sensor'}(t)$, 
Initially, $w_{\sensor}(0) = 1$ and $W_{\sensor}(0) = \numsensors$ for all $\sensor$. 
The central server stores $W(t)$ for all previous rounds $t$.
Let 
$\rho(w, W) := (1-\gamma)\frac{w}{W} + \frac{\gamma}{\numsensors}$.
Each sensor then proceeds with the sampling procedure of
section~\ref{sec:sampling} as though its probability mass in round $t$
was $q_{\sensor} = \rho(w_{\sensor}(t), W_{\sensor}(t))$ instead of its true
value of $\rho(w_{\sensor}(t), W(t))$.  Moreover, $\sensor$'s estimate 
$W_{\sensor}(t)$ is only updated on rounds when it communicates with
the server under these circumstances.  This allows the estimated
probabilities of all of the sensors to sum to more than one, but has
the benefit of significantly reducing the communication cost in the
star network model under certain assumptions.  
The protocol for round $t$ is as follows.

\begin{center}
\begin{tabular}{|p{8cm}|}
\hline
\textbf{The \LimitProtocol($\alpha$) with renormalization:}\\
\hspace{0cm} \emph{Sensors:} \\
\hspace{0cm} For each sensor $\sensor$ in parallel\\
\hspace{0.5cm} Sample $r_{\sensor}$ uniformly at random from $[0,1]$.\\
\hspace{0.5cm} If $(r_{\sensor} \ge 1 - \alpha \cdot \rho(w_{\sensor}(t), W_{\sensor}(t))$\\
\hspace{1cm} Send $\tuple{r_{\sensor}, w_{\sensor}(t)}$ to the server.\\ 
\hspace{1cm} Receive message $\tuple{a, b}$ from server.\\
\hspace{1cm} Set $W_{\sensor}(t+1) = a$, $w_{\sensor}(t+1) = b$. \\
\hspace{0.5cm} Else\\
\hspace{1cm} Set $W_{\sensor}(t+1) = W_{\sensor}(t)$, $w_{\sensor}(t+1) = w_{\sensor}(t)$.\\
%
\hspace{0cm} \emph{Server:}\\
\hspace{0cm} Receive messages from a set $S$ of sensors. \\
\hspace{0cm} If $S = \emptyset$, select nothing and wait for next round.\\
\hspace{0cm} Else\\
\hspace{0.5cm} For each sensor $\sensor \in S$\\
\hspace{1cm} Set $Y_{\sensor} = \min \set{x : \prob{X \le x} \ge r_{\sensor}}$, \\
\hspace{1cm} where $X \sim \Poisson{\alpha \cdot \rho(w_{\sensor}(t),W(t))}$.\\
%
%
%
\hspace{1cm} Select $\sensor$ with probability
$Y_{\sensor}/\sum_{\sensor' \in S} Y_{\sensor'}$.\\
\hspace{0.5cm} Observe the payoff for the selected sensor and\\
\hspace{0.5cm} compute $W(t+1)$ and $w_{\sensor}(t+1)$ for each
$\sensor \in S$\\
\hspace{0.5cm} using the \EXPthree update rule.\\
\hspace{0.5cm} For each $\sensor \in S$, send $\tuple{W(t+1), w_{\sensor}(t+1)}$ to $\sensor$.\\
\hline
\end{tabular}
\end{center}


We now describe the assumptions that allow lazy renormalization to
have low communication costs.
Fix an action $\sensor$ and a multiarmed bandit algorithm.
Let $p_{\sensor}(t) \in [0,1]$ be random variables denoting the
probability the algorithm assigns to $\sensor$ on round $t$.
The value of $p_{\sensor}(t)$ depends on the random choices made by
the algorithm and the payoffs observed by it on previous rounds.
We assume the following about $p_{\sensor}(t)$.
\begin{enumerate}
\item $p_{\sensor}(t)$ can be computed from local information
  $\sensor$ possesses and global information the server has.
\item There exists an $\epsilon > 0$ such that $p_{\sensor}(t)
  \ge \epsilon$ for all $t$.
\item $p_{\sensor}(t) < p_{\sensor}(t+1)$ implies $\sensor$ was
  selected in round $t$.
\item There exists $\hat{\epsilon} > 0$ such that 
  $p_{\sensor}(t+1) \ge p_{\sensor}(t)/(1+\hat{\epsilon})$ for all $t$.
\end{enumerate}
Many MAB algorithms satisfy these conditions.
For example, it is not too difficult to show \EXPthree does so 
with $\epsilon = \gamma/\numsensors$ and
$\hat{\epsilon} = (e-1)\frac{\gamma}{\numsensors}$, assuming payoffs in $[0,1]$.
In this case, Theorem~\ref{thm:lazy_renorm_ratio} bounds the expected
increase in sensor communications due to lazy renormalization.
%
%
%

\begin{theorem} \label{thm:lazy_renorm_ratio}
Fix a multiarmed bandit instance with possibly adversarial payoff
functions, and a MAB algorithm 
%
satisfying the above assumptions on its distribution over actions
$\set{p_{\sensor}(t)}_{\sensor \in \sensors}$.
Let $q_{\sensor}(t)$ be the corresponding random estimates for
$p_{\sensor}(t)$ maintained under lazy renormalization with
oversampling parameter $\alpha$.
Then for all $\sensor$ and $t$, 
\[
\E{q_{\sensor}(t)/p_{\sensor}(t)} \le 1 + \frac{\hat{\epsilon}}{\alpha\epsilon}
\]
and 
\[
\E{q_{\sensor}(t)} \le \paren{1 +
  \frac{\hat{\epsilon}}{\alpha\epsilon}} \E{p_{\sensor}(t)}
\mbox{.}
\]
\end{theorem}


\begin{proof}
Fix $\sensor$, and let $p(t) := p_{\sensor}(t)$, $q(t) := q_{\sensor}(t)$.
We begin by bounding $\prob{q(t) \ge \lambda p(t)}$ for $\lambda \ge
1$.  Let $t_0$ be the most recent round in which $q(t_0) = p(t_0)$.
We assume $q(0) = p(0)$, so $t_0$ exists.
Then $q(t) = p(t_0) \ge \lambda p(t)$  implies $p(t_0)/p(t)
\ge \lambda$.  By assumption $p(t')/p(t'+1) \le (1+\hat{\epsilon})$
for all $t'$, so $p(t_0)/p(t) \le (1+\hat{\epsilon})^{t-t_0}$.
Thus $\lambda \le (1+\hat{\epsilon})^{t-t_0}$ and 
$t-t_0 \ge \ln(\lambda)/ \ln (1+\hat{\epsilon})$. 
Define $t(\lambda) := \ln(\lambda)/ \ln (1+\hat{\epsilon})$.


By definition of $t_0$, there were no activations under lazy renormalization in rounds $t_0$
through $t-1$ inclusive, which occurs with probability 
$\prod_{t' = t_0}^{t-1} (1-\alpha q(t'))$ $=$ $(1-\alpha
q(t))^{t-t_{0}} $ $\le$ $(1-\alpha q(t))^{\ceil{t(\lambda)}}$, where $\alpha$ is the
oversampling parameter in the protocol.  
%
%
We now bound $\Econd{q(t)/p(t)}{q(t)}$.
Recall that $\E{X} = \int_{x = 0}^{\infty} \prob{X \ge x}dx$ for any non-negative
random variable $X$.  It will also be convenient to define 
$\lamexp := \ln(1/(1 - \alpha q(t))) / \ln(1+\hat{\epsilon})$ and assume for now
that $\lamexp > 1$.
Conditioning on $q(t)$, we see that 
\[
\begin{array}{lcl}
 \vspace{2mm}
\Econd{q(t)/p(t)}{q(t)} & = & \int_{\lambda = 0}^{\infty} \prob{q(t) \ge
  \lambda p(t)}d\lambda \\ 
 \vspace{2mm}
  & = & 1 + \int_{\lambda = 1}^{\infty} \prob{q(t) \ge
  \lambda p(t)}d\lambda \\ 
\vspace{2mm}
 & \le & 1 + \int_{\lambda = 1}^{\infty} (1-\alpha q(t))^{t(\lambda)}d\lambda\\
 \vspace{2mm}
 & = & 1 + \int_{\lambda = 1}^{\infty}
\lambda^{\ln(1-\alpha q(t))/\ln(1+\hat{\epsilon}) }d\lambda \\
 \vspace{2mm}
 & = & 1 + \int_{\lambda = 1}^{\infty} \lambda^{-\lamexp}d\lambda \\ 
 \vspace{2mm}
 & = & 1 + \frac{1}{\lamexp - 1}
%
%
\end{array}
\]
Using $\ln\paren{\frac{1}{1-x}} \ge x$ for all $x < 1$ and 
$\ln(1+x) \le x$ for all $x > -1$, we can show that 
%
%
$\lamexp \ge \alpha q(t)/\hat{\epsilon}$
so $1+\frac{1}{\lamexp - 1} \le \alpha
q(t)/(\alpha q(t) - \hat{\epsilon})$.
Thus, if $\alpha q(t) > \hat{\epsilon}$ then $\lamexp > 1$ and we
obtain 
$\Econd{q(t)/p(t)}{q(t)} \le  \alpha q(t)/(\alpha q(t) - \hat{\epsilon})$.


If $q(t) >> \hat{\epsilon}$, this gives a good bound.  If $q(t)$ is small, we
rely on the assumption that $p(t) \ge \epsilon$ for all $t$ to get a trivial
bound of $q(t)/p(t) \le q(t)/\epsilon$.
We thus conclude 
\begin{equation} \label{eqn:ratio-bound}
\Econd{q(t)/p(t)}{q(t)} \le \min \paren{\alpha q(t)/(\alpha q(t) - \hat{\epsilon}) ,\ q(t)/\epsilon}\mbox{.}
\end{equation}
Setting $q(t) = (\hat{\epsilon}/\alpha + \epsilon)$ to maximize this
quantity yields an unconditional bound of 
%
%
$\E{q(t)/p(t)} \le 1 + \hat{\epsilon}/\alpha\epsilon$.


To bound $\E{q(t)}$ in terms of $\E{p(t)}$, note that for all $q$
\begin{align*}
q/\Econd{p(t)}{q(t)=q} & \le \Econd{q(t)/p(t)}{q(t)=q}\\
                    & \le 1 + \hat{\epsilon}/\alpha\epsilon
\end{align*}
where the first line is by Jensen's inequality, and the second is by 
equation~\ref{eqn:ratio-bound}.
Thus $q \le \paren{1 +
  \hat{\epsilon}/\alpha\epsilon}\Econd{p(t)}{q(t)=q}$ for all $q$.
Taking the expectation with respect to $q$ then proves 
$\E{q_{\sensor}(t)} \le \paren{1 +
  \frac{\hat{\epsilon}}{\alpha\epsilon}} \E{p_{\sensor}(t)}$
as claimed.
\end{proof}


\begin{cor}
If \EXPthree is used with payoffs in $[0,1]$ then
$\E{q_{\sensor}(t)/p_{\sensor}(t)} \le 1 + (e-1)/\alpha$, and in
expectation at most $\alpha\paren{1 + (e-1)/\alpha}$ sensors activate
in any round $t$.
\end{cor}

\begin{proof}
We prove in Lemma~\ref{lem:exp3conditions} that \EXPthree satisfies
the conditions with $\epsilon = \gamma/\numsensors$ and $\hat{\epsilon} =
(e-1)\frac{\gamma}{\numsensors}$, which implies the first part of the
corollary.
For the second part, note that 
$\E{\sum_{\sensor} q_{\sensor}(t)} \le \paren{1 +
  (e-1)/\alpha}\E{\sum_{\sensor} p_{\sensor}(t)} = \paren{1 +
  (e-1)/\alpha}$, because $\sum_{\sensor} p_{\sensor}(t) = 1$.
Sensor $\sensor$ activates with probability $\alpha q_{\sensor}(t)$,
so the expected number of activations is 
$\E{\alpha \sum_{\sensor} q_{\sensor}(t)} \le \alpha\paren{1 + (e-1)/\alpha}$.
\end{proof}

Finally, it is not too difficult to show that lazy renormalization
selects each sensor $\sensor$ with probability
$(1-e^{-\alpha})p_{\sensor}(t)$, because of the way the random bits
$r_{\sensor}$ are shared in order to implement a coupled distribution for
sensor activation and selection.


\subsection{Distributed Selection} \label{sec:distributed-selection-single-sensor}

We are now ready to prove Theorem~\ref{thm:distributed-single-sensor-selection}.
Using the distributed multinomial sampling scheme with the lazy
renormalization scheme for \EXPthree with a fixed $\alpha$ 
we obtain a variant that selects each sensor $\sensor$ with
probability $(1-e^{-\alpha})p_{\sensor}(t)$, and nothing with
probability $e^{-\alpha}$.  
Since the rounds in which we select nothing are independent of the
payoffs, the total regret from these rounds is $\OPT e^{-\alpha}$ in
expectation.  For the other rounds, the standard regret bounds from
\EXPthree hold.  The total worst case bound on expected regret is thus 
$O(\sqrt{\OPT \numsensors \log \numsensors}$ $+$ $\OPT e^{-\alpha})$.
For the second half of the theorem statement, we can use the same idea
as in Theorem~\ref{thm:sampling};  that is, we can set 
$\alpha = c \ln \numsensors$ with $c \ge 1$, and in the rare event that no sensors
activate in a round, broadcast a signal to all of the sensors to rerun
the protocol, repeating as often as needed.  The resulting
distribution on sensor selections is precisely the same as in
\EXPthree. 
Since two processes are indistinguishable from the vantage point of
the (possibly adversarial) environment, the same regret bounds hold.

}


%
%
%
%
%
%

